Stochastic Shortest Path: Minimax, Parameter-Free and Towards Horizon-Free Regret

We study the problem of learning in the stochastic shortest path (SSP) setting, where an agent seeks to minimize the expected cost accumulated before reaching a goal state. We design a novel model-based algorithm EB-SSP that carefully skews the empirical transitions and perturbs the empirical costs with an exploration bonus to induce an optimistic SSP problem whose associated value iteration scheme is guaranteed to converge. We prove that EB-SSP achieves the minimax regret rate $\tilde{O}(B_{\star} \sqrt{S A K})$, where $K$ is the number of episodes, $S$ is the number of states, $A$ is the number of actions, and $B_{\star}$ bounds the expected cumulative cost of the optimal policy from any state, thus closing the gap with the lower bound. Interestingly, EB-SSP obtains this result while being parameter-free, i.e., it does not require any prior knowledge of $B_{\star}$, nor of $T_{\star}$, which bounds the expected time-to-goal of the optimal policy from any state. Furthermore, we illustrate various cases (e.g., positive costs, or general costs when an order-accurate estimate of $T_{\star}$ is available) where the regret only contains a logarithmic dependence on $T_{\star}$, thus yielding the first (nearly) horizon-free regret bound beyond the finite-horizon MDP setting.

==> 6-conclusion.tex <==
\section{Conclusion}\label{sect_conclusion}


In this paper, we introduced \ALGO, an algorithm for online SSP with the two following important properties. \textbf{1)}~It is the first algorithm that is \textit{simultaneously} nearly minimax-optimal and parameter-free (i.e., it does not require to know $T_{\star}$ nor $B_{\star}$). \textbf{2)}~In various cases its regret can be coined ``horizon-free'' since it only has a \textit{logarithmic} dependence on $T_{\star}$, thus exponentially improving over existing bounds in terms of the dependence on $T_{\star}$, which may be arbitrarily larger than $B_{\star}$ in SSP models with small instantaneous costs. 

Beyond our improvements in the SSP setting, we can highlight two broader implications of our results. \textbf{1)}~We show that it is possible to devise an adaptive exploration bonus strategy in a setting where no prior knowledge of the ``optimal range'' is available (this was an open question raised in \citet{jian2019exploration} whose exploration-bonus-based approach in average-reward MDPs requires prior knowledge of the optimal bias span). \textbf{2)}~We show that the concept of horizon-free regret can be extended beyond finite-horizon MDPs \citep[e.g.,][]{wang2020long, zhang2020reinforcement,zhang2021variance}. In fact, it is perhaps even more meaningful in the goal-oriented setting, by virtue of the already present distinction between ``optimal length'' ($T_{\star}$) and ``optimal return'' ($B_{\star}$). Indeed we do not make any extra assumption on the SSP problem, as opposed to the finite-horizon set-up which requires the assumption of different episode length ($H$) and episode return of \textit{any} trajectory (at most~$1$) so as to uncover horizon-free properties. 

An interesting question raised by our paper is whether it is possible to simultaneously achieve the three properties of minimax, parameter-free and horizon-free regret for SSP under general costs. Another interesting direction would be to build on our approach (e.g., the \VISGO procedure) to derive tight sample complexity bounds in SSP, which as explained in \citet{tarbouriech2021sample} do not directly ensue from regret guarantees.


==> checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We provide open questions and directions for future investigation in the conclusion of the paper.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{This paper makes contributions to the fundamentals of online learning (RL) and due to its theoretical nature, we see no ethical or immediate societal consequence of our work.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
